InstructEdit: Instruction-based Knowledge Editing for Large Language Models

Knowledge editing for large language models can offer an efficient solution to alter a model's behavior without negatively impacting the overall performance. However, the current approaches encounter issues with limited generalizability across tasks, necessitating one distinct editor for each task, significantly hindering the broader applications. To address this, we take the first step to analyze the multi-task generalization issue in knowledge editing. Specifically, we develop an instruction-based editing technique, termed InstructEdit, which facilitates the editor's adaptation to various task performances simultaneously using simple instructions. With only one unified editor for each LLM, we empirically demonstrate that InstructEdit can improve the editor's control, leading to an average 14.86% increase in Reliability in multi-task editing setting. Furthermore, experiments involving holdout unseen task illustrate that InstructEdit consistently surpass previous strong baselines. To further investigate the underlying mechanisms of instruction-based knowledge editing, we analyze the principal components of the editing gradient directions, which unveils that instructions can help control optimization direction with stronger OOD generalization. Code and datasets are available in https://github.com/zjunlp/EasyEdit.

==> delete/todo.tex <==
% - Model Editing...那节中的定义与Instruction Editing...是否需要对应 (符号保持一致)
% - 公式丰富 (参考姚博EMNLP2023问题定义)
% - Editor的定义 (background，参考MEND加上超网络的公式，定义朝梯度靠近)
% - `Instruction Editing Task Definitions` 这个标题似乎有点不合适。这个section中没有instruction相关内容 
- Instruction Example (正文一定要有)
- Dataset stat (table 2) 在正文中没有引用 (在数据集部分引入)
% - 'Examples of these descriptions are provided in Table 3' 这个描述可以接在`Description`定义后面
- （Optional）多任务设置有点问题，为什么一定是 Train {CF, ConvSent, Recent}, Test {ZsRE}，是否需要加一组其他组合
- Table 4: Main results中`Multi-Task Editing`标题是否不合适，其他方法也是Multi-Task Training？ 如果是，需要在`Experimental Setting`中有相关说明，如果不是，也同样要说明baseline方法都是在Single-task training的结果；总的说来，可以更多些实验细节（比如训练上的setting）
- Multi-task Editing Results中baseline的performance描述过多，而且缺乏baseline与InstructEdit的比较；如第一段FT-L的results，可以直接加与InstructEdit的比较，后同；感觉可以针对每种baseline方法，凝练一个突出的缺陷（如在某个metric上效果很差，加一个解释），拿InstructEdit的优势去打这个点；

% - task num performance的表
% - convsent实验补全
% - pilot实验表格补全
% - 图5 caption完成
% - exact match performance alter

==> tab/dataset.tex <==
\begin{table}[!b]
% \setlength{\tapcolsep}{4cm}
\centering
\small
\resizebox{1.0\columnwidth}{!}{
\resizebox{0.5\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{lcccccccc}
\toprule
              % &         \multicolumn{4}{c}{\bf FB15k-237}                           &        \multicolumn{4}{c}{\bf WN18RR}                           \\ \cmidrule(lr){2-5}                         \cmidrule(lr){6-9}   
Type  & \wikicf & \wikirecent & \convsent & \zsre \\
\midrule
% \rule{0pt}{15pt}
Train     & 1,427 & 570 & 14,390 & - \\
% \rule{0pt}{15pt}
Test    &  839 & 1,266 & 800 & 1,037 \\
\bottomrule
\end{tabular}
}%
}
\caption{
The statistics of datasets.
}
\label{tab:dataset}
\end{table}

==> tab/main_results_bak.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{table*}[ht]
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
\small
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|c|ccc|ccc}
% \hline
\toprule
\textbf{DataSet}     & \textbf{Model}                                      & \textbf{Metric}   &  \textbf{Base} & $\textbf{GRACE}$
& $\textbf{FT-L}$ & $\textbf{CaliNet}$ & $\textbf{KE}$
& $\textbf{MEND}$ & $\textbf{InstructEdit}$  \\ 
\midrule
\multirow{7}{*}{\textbf{\wikicf}}        & \multirow{3}{*}{GPT2-XL}                    
& Reliability & 18.06  & 29.14 & 21.41 & 23.41 & 88.96 & 71.87 & 89.62  \\
&

& Generality & 18.72  & 17.62 & 2.04 & 21.34 & 74.80 & 64.13 & 73.00  \\
                             &                                           
& Locality & 100.0 & 39.95 & 21.93 & 60.83 & 62.14 & 82.51 & 87.07  \\
                             &                                           
& Portability & 11.00 & 11.57 & 7.36 & 12.40 & 41.99 & 31.75 & 45.98 \\ 
\cmidrule{2-10} 
                             & \multirow{3}{*}{LLaMA-2}                     
& Reliability & 27.01  & 47.38 & 14.98 & 22.53 & 94.22 & 93.03 & 96.23 \\
&

& Generality & 26.97  & - & - & - & 78.97 & 76.13 & 86.63  \\
                             &                                           
& Locality & 100.0 & 32.04 & 54.49 & 32.38 & 83.49 & 88.12 & 95.37 \\
                             &                                           
& Portability & 27.04 & 35.35 & 3.75 & 9.44 & 63.60 & 61.61 & 62.61 \\ 

\midrule
\multirow{7}{*}{\textbf{\wikirecent}} & \multirow{3}{*}{GPT2-XL}                    
& Reliability & 28.95  & 55.25 & 39.00 & 41.05 & 97.18 & 84.51 & 92.64 \\
&

& Generality & 28.28  & 33.60 & 7.39 & 39.70 & 66.74 & 69.25 & 73.27  \\
                             &                                           
& Locality & 100.0 & 45.73 & 26.58 & 59.00 & 80.69 & 71.78 & 81.04 \\
                             &                                           
& Portability & 17.19 & 23.56 & 16.78 & 21.34 & 40.68 & 37.23 & 43.85 \\ 
\cmidrule{2-10} 
                             & \multicolumn{1}{c}{\multirow{3}{*}{LLaMA-2}} 
& Reliability & 50.16  & 58.66 & 23.52 & 21.97 & 97.19 & 96.13 & 96.17 \\
&

& Generality & 46.38  & - & - & - & 66.19 & 81.48 & 91.75  \\
                             &                                           
& Locality & 100.0 & 35.05 & 59.74 & 50.56 & 97.31 & 83.74 & 94.18 \\
                             &                                           
& Portability & 43.52 & 41.77 & 7.08 & 11.52 & 59.24 & 60.93 & 62.61 \\ 

\midrule

\multirow{3}{*}{\textbf{\convsent}} & \multirow{3}{*}{GPT2-XL}                    
& Reliability & -  & 48.93 & 50.41 & 49.52 & 49.77 & 54.98 & 49.13 \\

                             &                                           
& Locality & 100.0 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 \\    
                            & 
& Fluency & - & 621.66 & 528.55 & 497.21 & 520.32 & 337.64 & 604.24 \\          

% \cmidrule{2-10} 
%                              & \multicolumn{1}{c}{\multirow{3}{*}{\textit{\textbf{Llama-2}}}} 
% & Edit Succ. & -  & - & - & - & - & - & - \\
%                              &                                           
% & Locality & - & - & - & - & - & - & - \\
%                             & 
% & Fluency & - & - & - & - & - & - & - \\

\midrule

\multicolumn{10}{c}{\textbf{\small Hold Out}} \\

\midrule

\multirow{7}{*}{\textbf{\zsre}} & \multirow{3}{*}{\textit{\textbf{GPT2-XL}}}                    
& Reliability & 24.92  & 56.05 & 0.11 & 0.86 & 97.11 & 69.30 & 97.51 \\
&

& Generality & 23.93  & 30.54 & 0.08 & 0.78 & 96.33 & 63.38 & 96.14  \\
                             &                                           
& Locality & 100.0 & 84.99 & 100.0 & 100.0 & 98.86 & 98.57 & 98.17 \\
                             &                                           
& Portability & 47.07 & 45.37 & 0.55 & 0.86 & 48.77 & 46.79 & 47.62 \\ 
\cmidrule{2-10} 
                             & \multicolumn{1}{c}{\multirow{3}{*}{\textit{\textbf{LLaMA-2}}}} 
& Reliability & 40.29  & 56.66 & 2.23 & 1.23 & 95.98 & 82.27 & 84.88 \\
&

& Generality & 39.43  & - & - & - & 93.73 & 73.44 & 80.06  \\
                             &                                           
& Locality & 100.0 & 96.35 & 100.0 & 100.0 & 99.52 & 97.97 & 99.27 \\
                             &                                           
& Portability & 56.66 & 55.13 & 0.54 & 1.17 & 57.69 & 57.69 & 57.62 \\ 
\bottomrule
\end{tabular}
}
}
\caption{Main results.}
\label{tab:main-results}  
\end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \newcommand\resulttablefontsize{\fontsize{7.7pt}{9.24pt}\selectfont}
% \newcommand{\first}[1]{%
%   \begingroup
%   \setlength{\fboxsep}{0pt}% 无内边距
%   \colorbox{blue!25}{#1}%
%   \endgroup
% }

% 2024.1.17
\newcommand{\first}{\colorbox{blue!25}}
\newcommand{\second}{\colorbox{blue!10}}
% \definecolor{Mycolor1}{HTML}{BAD8F2}
% \definecolor{Mycolor2}{HTML}{DDEEFA}
\begin{table*}[t]
{
% \renewcommand{\arraystretch}{1.15}
% \setlength{\tabcolsep}{3pt}
% \small
% \resulttablefontsize
\resizebox{\textwidth}{!}{
\begin{tabular}{lcc|c|ccccc|c}
% \hline
\toprule
\textbf{DataSet}     & \textbf{Model}                                      & \textbf{Metric}   &  \textbf{Base} 
& $\textbf{FT-L}$ & $\textbf{CaliNet}$ & $\textbf{KE}$
& $\textbf{MEND}$ & $\textbf{GRACE}$   & $\textbf{InstructEdit}$  \\ 
\midrule
\multicolumn{10}{c}{\textbf{\small Multi-Task Editing}} \\
\midrule
\multirow{7}{*}{\textbf{\wikicf}}        & \multirow{3}{*}{GPT2-XL}                  
& Reliability   & 0.00 & 0.40 & 0.24 & 33.97 & \underline{74.26} & 0.00 & \textbf{80.81}  \\
&

& Generalization   & 0.00 & 0.32 & 0.12 & 8.70 & \underline{46.48} & 0.00 & \textbf{53.16}  \\
                             &                                           
& Locality   & 100.0 & 43.73 & 82.81 & \underline{90.94} & 58.68 & \textbf{100.0} & 67.83  \\
                             &                                           
& Portability   & 11.00 & 0.87 & 3.64 & 27.41 & \underline{41.88} & 11.00 & \textbf{50.83} \\ 
\cmidrule{2-10} 
                             & \multirow{3}{*}{LLaMA-2}                     
& Reliability   & 0.00 & 0.00 & 0.00 & 2.98 & \underline{84.15} & 0.00 & \textbf{84.39} \\
&

& Generalization   & 0.00 & 0.00 & 0.00 & 0.00 & \underline{44.10} & 0.00 & \textbf{50.18}  \\
                             &                                           
& Locality   & 100.0 & 70.66 & 89.28 & 90.86 & \underline{91.18} & \textbf{100.0} & 88.04 \\
                             &                                           
& Portability   & 27.04 & 3.19 & 26.93 & 33.43 & \underline{65.84} & 27.04 & \textbf{69.43} \\ 

\midrule
\multirow{7}{*}{\textbf{\wikirecent}} & \multirow{3}{*}{GPT2-XL}                    
& Reliability   & 2.61 & 6.48 & 11.53 & 49.37 & \underline{85.62} & 2.61 & \textbf{85.70} \\
&

& Generalization   & 1.58 & 2.21 & 5.37 & 10.98 & \textbf{52.76} & 1.58 & \underline{51.66}  \\
                             &                                           
& Locality   & 100.0 & 26.58 & 83.87 & \underline{87.12} & 57.94 & \textbf{100.0} & 64.61 \\
                             &                                           
& Portability   & 17.19 & 16.78 & 10.31 & 30.41 & \underline{42.26} & 17.19 & \textbf{47.36} \\ 
\cmidrule{2-10} 
                             & \multicolumn{1}{c}{\multirow{3}{*}{LLaMA-2}} 
& Reliability   & 9.87 & 6.16 & 9.79 & 15.88 & \underline{82.31}  & 9.87 & \textbf{83.73} \\
&

& Generalization   & 7.27  & 3.87 & 6.64 & 0.08 & \underline{54.66} & 7.27 & \textbf{55.92}  \\
                             &                                           
& Locality   & 100.0 & 70.66 & \underline{89.28} & 88.88 & 78.57 & \textbf{100.0} & 87.04 \\
                             &                                           
& Portability   & 43.52 & 3.15 & 43.26 & 43.52 & \underline{60.84} & 43.52 & \textbf{62.39} \\ 

\midrule

\multirow{3}{*}{\textbf{\convsent}} & \multirow{3}{*}{GPT2-XL}                    
& Reliability   & 40.74 & 7.48 & 37.47 & 53.07 & \underline{54.67}  & 40.74 & \textbf{65.43} \\

                             &                                           
& Locality   & 100.0 & 42.86 & 87.47 & 94.58 & \underline{96.58} & \textbf{100.0}  & 94.27 \\    
                            & 
& Fluency   & 613.13 & 548.55 & 396.43 & \underline{615.61} & 601.93 & 613.13 & \textbf{617.65} \\          

% \cmidrule{2-10} 
%                              & \multicolumn{1}{c}{\multirow{3}{*}{\textit{\textbf{Llama-2}}}} 
% & Edit Succ. & -  & - & - & - & - & - & - \\
%                              &                                           
% & Locality & - & - & - & - & - & - & - \\
%                             & 
% & Fluency & - & - & - & - & - & - & - \\

\midrule

\multicolumn{10}{c}{\textbf{\small Hold Out Editing}} \\

\midrule

\multirow{8}{*}{\textbf{\zsre}} & \multirow{4}{*}{GPT2-XL}                    
& Reliability   & 0.00 & 0.11 & 0.00 & 13.50 & \underline{40.79}  & 0.00 & \textbf{82.83} \\
&

& Generalization   & 0.00 & 0.08 & 0.10 & 10.13 & \underline{31.15}  & 0.00 & \textbf{78.40}  \\
                             &                                           
& Locality   & 100.0 & 74.06 & \underline{95.66} & 82.59 & 94.79 & \textbf{100.0} & 94.57 \\
                             &                                           
& Portability   & 47.07 & 0.96 & 0.39 & 43.90 & \underline{45.08} & \textbf{47.07} & 40.84 \\ 
\cmidrule{2-10} 
                             & \multicolumn{1}{c}{\multirow{4}{*}{LLaMA-2}} 
& Reliability   & 0.00 & 2.23 & 0.00 & 2.70 & \textbf{76.95}  & 0.00 & \underline{76.57} \\
&

& Generalization   & 0.00 & 1.93 & 0.00 & 0.19 & \underline{67.89}  & 0.00 & \textbf{70.11}  \\
                             &                                           
& Locality   & 100.0 & 98.89 & \underline{99.66} & 95.15 & 90.14 & \textbf{100.0} & 94.16 \\
                             &                                           
& Portability   & 56.66 & 0.54 & 0.87 & 48.02 & \textbf{58.63} & 56.66 & \underline{58.19} \\ 
\bottomrule
\end{tabular}
}
}
\caption{Main results. All metrics are designed with higher values indicating superior performance.}
\label{tab:main-results}  
\end{table*}
% \begin{table*}[ht]
% {
% % \renewcommand{\arraystretch}{1.15}
% % \setlength{\tabcolsep}{3pt}
% \small
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcc|c|ccc|ccc|c}
% % \hline
% \toprule
% \textbf{DataSet}     & \textbf{Model}                                      & \textbf{Metric}   &  \textbf{Base} & $\textbf{FT-L}_\text{Single}$
% & $\textbf{FT-L}_\text{Multi}$ & $\textbf{FT-L}_\text{Instruct}$ & $\textbf{MEND}_\text{Single}$
% & $\textbf{MEND}_\text{Multi}$ & $\textbf{MEND}_\text{Instruct}$  &
% $\textbf{Editor}_\text{Instruct}$\\ 
% \midrule
% \multirow{7}{*}{\textbf{\wikicf}}        & \multirow{3}{*}{GPT2-XL}                    
% & Edit Succ. & 18.06  & 28.95 & 21.48 & 22.34 & - & 71.87 & 86.58 \\
%                              &                                           
% & Locality & 100.0 & 40.19 & 21.95 & 57.70 & - & 82.51 & 86.09 \\
%                              &                                           
% & Portability & 11.00 & 11.69 & 7.36 & 1.12 & - & 31.75 & 30.53 \\ 
% \cmidrule{2-10} 
%                              & \multirow{3}{*}{Llama-2}                     
% & Edit Succ. & 27.01  & 47.38 & 14.98 & 22.53 & 78.82 & 93.03 & 95.73 \\
%                              &                                           
% & Locality & 100.0 & 32.04 & 54.49 & 32.38 & 94.16 & 88.12 & 95.35 \\
%                              &                                           
% & Portability & 27.04 & 35.35 & 3.75 & 9.44 & 57.53 & 61.61 & 45.33 \\ 

% \midrule
% \multirow{7}{*}{\textbf{\wikirecent}} & \multirow{3}{*}{GPT2-XL}                    
% & Edit Succ. & 28.95  & 55.28 & 39.06 & 41.16 & - & 84.51 & 92.35 \\
%                              &                                           
% & Locality & 100.0 & 45.82 & 26.57 & 57.56 & - & 71.78 & 79.38 \\
%                              &                                           
% & Portability & 17.19 & 23.33 & 16.78 & 4.60 & - & 37.23 & 30.81 \\ 
% \cmidrule{2-10} 
%                              & \multicolumn{1}{c}{\multirow{3}{*}{Llama-2}} 
% & Edit Succ. & 50.16  & 58.66 & 23.52 & 21.97 & 76.88 & 96.13 & 96.17 \\
%                              &                                           
% & Locality & 100.0 & 35.05 & 59.74 & 50.56 & 92.87 & 83.74 & 94.18 \\
%                              &                                           
% & Portability & 43.52 & 41.77 & 7.08 & 11.52 & 50.11 & 60.93 & 48.79 \\ 

% \midrule

% \multirow{5}{*}{\textbf{\convsent}} & \multirow{2}{*}{GPT2-XL}                    
% & Edit Succ. & -  & - & - & - & - & 54.98 & 49.04 \\
%                              &                                           
% & Locality & - & - & - & - & - & 0.00 & 0.00 \\          

% \cmidrule{2-10} 
%                              & \multicolumn{1}{c}{\multirow{2}{*}{\textit{\textbf{Llama-2}}}} 
% & Edit Succ. & -  & - & - & - & - & - & - \\
%                              &                                           
% & Locality & - & - & - & - & - & - & - \\

% \midrule

% \multirow{7}{*}{\textbf{\zsre}} & \multirow{3}{*}{\textit{\textbf{GPT2-XL}}}                    
% & Edit Succ. & 24.92  & 56.14 & 0.11 & 0.99 & - & 69.30 & 96.32 \\
%                              &                                           
% & Locality & 100.0 & 85.65 & 100.0 & 100.0 & - & 98.57 & 98.06 \\
%                              &                                           
% & Portability & 47.07 & 45.47 & 0.55 & 0.56 & - & 46.79 & 47.95 \\ 
% \cmidrule{2-10} 
%                              & \multicolumn{1}{c}{\multirow{3}{*}{\textit{\textbf{Llama-2}}}} 
% & Edit Succ. & 40.29  & 56.66 & 2.23 & 1.23 & - & 82.27 & 84.88 \\
%                              &                                           
% & Locality & 100.0 & 96.35 & 100.0 & 100.0 & - & 97.97 & 99.27 \\
%                              &                                           
% & Portability & 56.66 & 55.13 & 0.54 & 1.17 & - & 57.69 & 57.62 \\ 
% \bottomrule
% \end{tabular}
% }
% }
% \caption{Main results.}
% \label{tab:main-results}  
% \end{table*}


==> tab/temp.tex <==
% \begin{table}
% \resizebox{\linewidth}{!}{
% \begin{NiceTabular}{llccc}
% \toprule
% Method  & &  ZsRE$ \Rightarrow$ Wiki$_{recent}$  &  Wiki$_{recent}$ $\Rightarrow$ Wiki$_{counterfact}$  &  Wiki$_{recent}$ $\Rightarrow$ ZsRE\\ \midrule
% \Block{4-1}{\textbf{MEND}} & Edit Succ. & 95.91 & 66.15 & 89.79 \\
% & Portability & 61.80 & 45.95 & 54.36 \\
% & Locality & 66.57 & 94.83 & 95.80 \\ 
% & Fluency & 554.28 & 592.82 & 571.39 \\
% \midrule
% \Block{4-1}{\textbf{SERAC}} & Edit Succ. & 97.42 & 99.43 & 99.31 \\
% & Portability & 60.42 & 68.85 & 57.70 \\
% & Locality & 27.25 & 100.00 & 79.04 \\
% & Fluency & 487.29 & 552.51 & 511.95 \\
%  \bottomrule
% \end{NiceTabular}
% }
% \caption{\textbf{Cross-Domain Edit Results.} 
% Performance (accuracy) of the compared methods, which are firstly trained on a source dataset and then directly conduct prediction on a target dataset (denoted as source $\Rightarrow$ target).}
% \label{tab:ood_results}
% \end{table}
\begin{table}
\centering
% \small
% \setlength{\tabcolsep}{0.8pt}
\resizebox{0.97\columnwidth}{!}{
% \resizebox{0.8\textwidth}{!}{
\begin{tabular}{cccccc}
\toprule
Source Domain & Target Domain & Reliability  & Generalization  &  Locality  & Portability  \\
\cmidrule{1-6}
\textbf{Recent Base} &  97.16  & 38.94  & 65.04  & 42.17 \\
\textbf{CounterFact} $\Rightarrow$ \textbf{Recent}    &  10.90$\downarrow$  & 14.37$\downarrow$  & 11.03$\downarrow$   & 13.04$\downarrow$  \\
\textbf{ZsRE} $\Rightarrow$ \textbf{Recent}    &  10.90$\downarrow$  & 14.37$\downarrow$  & 11.03$\downarrow$   & 13.04$\downarrow$  \\
\cmidrule{1-6}
\textbf{CounterFact Base} &  84.62 & 46.01 & 61.93 & 42.46\\
\cmidrule{1-6}
\textbf{Recent} $\Rightarrow$ \textbf{CounterFact} &  25.50$\downarrow$  & 33.40$\downarrow$  & 18.49$\downarrow$   & 16.59$\downarrow$ \\
\textbf{ZsRE} $\Rightarrow$ \textbf{CounterFact}    &  18.91$\downarrow$  & 14.80$\downarrow$  & 17.87$\downarrow$   & 18.16$\downarrow$ \\

\cmidrule{1-6}
\textbf{ZsRE Base} & 96.62 & 94.60 & 99.27 & 48.85 \\
\cmidrule{1-6}
\textbf{CounterFact} $\Rightarrow$ \textbf{ZsRE}    &  18.91$\downarrow$  & 14.80$\downarrow$  & 17.87$\downarrow$   & 18.16$\downarrow$ \\
\textbf{Recent} $\Rightarrow$ \textbf{ZsRE}    &  29.16$\downarrow$  & 34.85$\downarrow$  & 12.55$\downarrow$   & 10.94$\downarrow$  \\
\bottomrule
\end{tabular}
}
\caption{Performance on zero-shot domain transfer. Transferring the Editor's editing domain can result in a significant decrease.}
\label{tab:ood_results}
\end{table}

==> tab/unseen_instruct.tex <==
\begin{table}[t]
% \setlength{\tapcolsep}{4cm}
\centering
\small
\resizebox{1.0\columnwidth}{!}{
\resizebox{0.5\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{lcccccccc}
\toprule
              % &         \multicolumn{4}{c}{\bf FB15k-237}                           &        \multicolumn{4}{c}{\bf WN18RR}                           \\ \cmidrule(lr){2-5}                         \cmidrule(lr){6-9}   
Metrics  & \wikicf & \wikirecent & \convsent & \zsre \\
\midrule
% \rule{0pt}{15pt}
Edit Succ.     & 95.60 & 95.64 & - & 84.04 \\
% \rule{0pt}{15pt}
Locality    &  95.08 & 93.87 & - & 99.22 \\
Portability    &  45.49 & 48.93 & - & 57.56 \\
\bottomrule
\end{tabular}
}
}
\caption{
The results of $\text{MEND}_{Instruct}$ with unseen instructions. (LLaMA-2)
}
\label{tab:unseen_instruct}
\end{table}
